Differentially Private Multi-objective Selection: Pareto and Aggregation Approaches

Differentially private selection mechanisms are fundamental building blocks for privacy-preserving data analysis. While numerous mechanisms exist for single-objective selection, many real-world applications require optimizing multiple competing objectives simultaneously. We present two novel mechanisms for differentially private multi-objective selection: PrivPareto and PrivAgg. PrivPareto uses a novel Pareto score to identify solutions near the Pareto frontier, while PrivAgg enables privacy-preserving weighted aggregation of multiple objectives. Both mechanisms support global and local sensitivity approaches, with comprehensive theoretical analysis showing how to compose sensitivities of multiple utility functions. We demonstrate the practical applicability through two real-world applications: cost-sensitive decision tree construction and multi-objective influential node selection in social networks. The experimental results showed that our local sensitivity-based approaches achieve significantly better utility compared to global sensitivity approaches across both applications and both Pareto and Aggregation approaches. Moreover, the local sensitivity-based approaches are able to perform well with typical privacy budget values $\epsilon \in [0.01, 1]$ in most experiments.

==> sections/50_privagg_old.tex <==
\section{PrivAgg Mechanism}
\label{sec:privagg}

We present PrivAgg mechanism, a multi-objective differentially private algorithm for selecting the best candidate from a set of solutions that maximize the aggregate of the multiple objective functions, denoted as the utility functions $u_1, \cdots , u_m$. 

In this approach, we aggregate the utility functions into a single utility function $u_{agg}(x,r)$. More specially, we define the aggregate utility function $u_{agg}(x,r)$ as the weighted sum of the utility functions $u_{agg} = \sum_{i=1}^{m} w_i \cdot u_i(x,r)$, where $w_i$ is the weight of the utility function $u_i$. The weights can be defined by the data querier. 

Therefore, the PrivAgg mechanism outputs the candidate $r$ that maximizes the aggregate utility function $u_{agg}(x,r)$. Like the PrivPareto mechanism (Section \ref{sec:privpareto}), it has two versions: a global sensitivity version and a local sensitivity version. The global sensitivity version is used when only the global sensitivities of the underlying utility functions $u_1, \cdots , u_m$ are known. Otherwise, the local sensitivity version is used.

The global sensitivity version of the PrivAgg mechanism is defined as follows:

\begin{definition}
    (PrivAgg Mechanism - Global Sensitivity). The global PrivAgg mechanism $PrivAgg_{global} (x, \epsilon, u_1, \ldots, u_m, \mathcal{R})$ takes as input a database $x \in \domain$, the privacy budget $\epsilon$, the utility functions $u_1, u_2, \ldots, u_m: \range \times \domain \rightarrow \real$, the set of candidate solutions $\range$, and outputs a candidate $r \in \range$. The mechanism is defined as follows:    
    $$ PrivAgg_{global}(x, \epsilon, u_1, \ldots, u_m, \mathcal{R}) = \mec_{global}(x, \epsilon, u_{agg},\Delta {u_agg}, \mathcal{R}) $$
    where $u_{agg}(x,r) = \sum_{i=1}^{m} w_i \cdot u_i(x,r)$ is the aggregate utility function, $\Delta u_{agg}$ is the global sensitivity of the aggregate utility function, and $\mec_{global}$ is a single objective differentially private mechanism.
\end{definition}

The local sensitivity version of the PrivAgg mechanism is defined as follows:


\begin{definition}
    (PrivAgg Mechanism - Local Sensitivity). The local PrivAgg mechanism $PrivAgg_{local} (x, \epsilon, u_1, \ldots, u_m, \delta^{u_1}, \ldots, \delta^{u_m}, \mathcal{R})$ takes as input a database $x \in \domain$, the privacy budget $\epsilon$, the set of utility functions $u_1, u_2, \ldots, u_m: \range \times \domain \rightarrow \real$, the admissible sensitivity functions $\delta^{u_1} , \ldots, \delta^{u_m}$ of the utility functions, a set of candidate solutions $\range$, and outputs a candidate $r \in \range$. The mechanism is defined as follows:
    \begin{multline}
        PrivAgg_{local} (x, \epsilon, u_1, \ldots, u_m, \delta^{u_1}, \ldots, \delta^{u_m}, \mathcal{R})  \\ = \mec_{local}(x, \epsilon, u_{agg}, \delta^{u_{agg}}, \mathcal{R})
    \end{multline}
\end{definition}

% In the next subsection we analyze the global sensitivity $\Delta {u_agg}$ of the aggregate utility function $u_{agg}$ and the local sensitivity $\delta^{u_{agg}}$ of the aggregate utility function $u_{agg}$.

\subsection{Sensitivity Analysis}

In this subsection, we discuss how to compute the global and local sensitivity for $u_{agg}$. First, we prove some base properties of admissible sensitivity functions regarding multiplication by a constant (Lemma \ref{teo:mult_const}) and sum of admissible functions (Lemma \ref{teo:sum_sens}).

\begin{lemma}
    (Multiplication by Constant). Let $u: \range \times \domain \rightarrow \real$ be a utility function, $\delta^u: \domain \times \range \times \range \rightarrow \real$ be an admissible sensitivity function of $u$ and $C$ a constant. Then    
    $$ \delta^{u.C}(x,t,r) = |C|.\delta^{u}(x,t,r) $$    
    is an admissible sensitivity function of $u.C$.
    \label{teo:mult_const}
\end{lemma}

\begin{proof}
    Let $u: \range \times \domain \rightarrow \real$ be a utility function, $\delta^u: \domain \times \range \times \range \rightarrow \real$ be an admissible sensitivity function of $u$ and $C$ a constant. We have that
    
    \begin{align*}
        \delta^{u.C}(x,t,r) & = \max_{r' \in \range} |C.u(x,r) - C.u(x,r')| \\
        & = \max_{r' \in \range} |C|.|u(x,r) - u(x,r')| \\
        & = |C|.\max_{r' \in \range} |u(x,r) - u(x,r')| \\
        & = |C|.\delta^{u}(x,t,r)
    \end{align*}
    
    Thus, $\delta^{u.C}(x,0,r) = |C|.\delta^{u}(x,0,r) \geq |C|.0 = 0$ and $\delta^{u.C}(x,t+1,r) = |C|.\delta^{u}(x,t+1,r) \geq |C|.\delta^{u}(y,t,r) = \delta^{u.C}(y,t,r)$, for all $t \geq 0$, $r \in \range$ and databases $x$ and $y$ s.t. $d(x,y) \leq 1$ as $\delta^{u}$ is admissible. Therefore, $\delta^{u.C}$ is an admissible sensitivity function of $u.C$.
\end{proof}


\begin{lemma}
    (Sum of Admissible Sensitivity Functions). Let $u: \range \times \domain \rightarrow \real$ be a utility function, $\delta^u: \domain \times \range \times \range \rightarrow \real$ and $\delta^{u'}: \domain \times \range \times \range \rightarrow \real$ be admissible sensitivity functions of $u$ and $u'$, respectively. Then

    $$ \delta^{u+u'}(x,t,r) = \delta^{u}(x,t,r) + \delta^{u'}(x,t,r) $$

    is an admissible sensitivity function of $u+u'$.
    \label{teo:sum_sens}
\end{lemma}

\begin{proof}
    Let $u: \range \times \domain \rightarrow \real$ be a utility function, $\delta^u: \domain \times \range \times \range \rightarrow \real$ and $\delta^{u'}: \domain \times \range \times \range \rightarrow \real$ be admissible sensitivity functions of $u$ and $u'$, respectively. We have that $\delta^{u+u'}(x,0,r) =  \delta^{u}(x,0,r) + \delta^{u'}(x,0,r) \geq 0$ since $\delta^{u}$ and $\delta^{u'}$ are admissible. Therefore we have

    \begin{align*}
        \delta^{u+u'}(x,t+1,r) &  = \delta^{u}(x,t+1,r) + \delta^{u'}(x,t+1,r) \\
        & \geq \delta^{u}(y,t,r) + \delta^{u'}(y,t,r) = \delta^{u+u'}(y,t,r)
    \end{align*}

    since $\delta^{u}$ and $\delta^{u'}$ are admissible. Therefore, $\delta^{u+u'}$ is an admissible sensitivity function of $u+u'$.
\end{proof}

In what follows, a direct result of lemmas \ref{teo:mult_const} and \ref{teo:sum_sens} are given:

\begin{corollary} 
    (Admissible Sensitivity of Weighted Sum). Let $u_1, \ldots, u_m: \range \times \domain \rightarrow \real$ be utility functions, $\delta^{u_1}, \ldots, \delta^{u_m}$ be admissible sensitivity functions, and $w_1, \ldots, w_m$ be weights. Then an admissible sensitivity of the aggregate utility function $u_{agg}(x,r)$ is given by

    $$ \delta^{u_{agg}}(x,t,r) = \sum_{i=1}^{m} |w_i|.\delta^{u_i}(x,t,r) $$

    where $\delta^{u_i}$ is the admissible sensitivity function of the utility function $u_i$.
    \label{cor:agg_sens}
\end{corollary}

Also, we have give upper bounds on the global sensitivity so that we can use the upper bound value safely to satisfy $\epsilon$-differential privacy:


\begin{theorem}
    (Upper Bound on the Global Sensitivity of Aggregate Utility Function). Let $u_1, \ldots, u_m: \range \times \domain \rightarrow \real$ be utility functions and $w_1, \ldots, w_m$ be weights. We have

    $$ \Delta u_{agg} \leq \sum_{i=1}^{m} |w_i|.\Delta u_i $$

    where $\Delta u_i$ is the global sensitivity of the utility function $u_i$.
    \label{teo:global_sens_agg}
\end{theorem}

\begin{proof}
    Let $u_1, \ldots, u_m: \range \times \domain \rightarrow \real$ be utility functions and $w_1, \ldots, w_m$ be weights. We have that

    \begin{align*}
        \Delta u_{agg} & = \max_{x,y \in \domain} \max_{r \in \range} |u_{agg}(x,r) - u_{agg}(y,r)| \\
        & = \max_{x,y \in \domain} \max_{r \in \range} \left| \sum_{i=1}^{m} w_i.u_i(x,r) - \sum_{i=1}^{m} w_i.u_i(y,r) \right| \\
        & = \max_{x,y \in \domain} \max_{r \in \range} \left| \sum_{i=1}^{m} w_i.(u_i(x,r) - u_i(y,r)) \right| \\
        & \leq \sum_{i=1}^{m} |w_i|.\max_{x,y \in \domain} \max_{r \in \range} |u_i(x,r) - u_i(y,r)| \\
        & = \sum_{i=1}^{m} |w_i|.\Delta u_i
    \end{align*}

    \label{teo:global_sens_agg}
\end{proof}


Note that the global sensitivity may be smaller than the upper bound given in Theorem \ref{teo:global_sens_agg} for specific known utility functions. This theorem gives a worst-case upper bound for any two functions.



